Gradient Methods with Online Scaling Part II. Practical Aspects

Part I of this work [Gao25] establishes online scaled gradient methods (OSGM), a framework that utilizes online convex optimization to adapt stepsizes in gradient methods. This paper focuses on the practical aspects of OSGM. We leverage the OSGM framework to design new adaptive first-order methods and provide insights into their empirical behavior. The resulting method, OSGM-Best, matches the performance of quasi-Newton variants while requiring less memory and cheaper iterations. We also extend OSGM to nonconvex optimization and outline directions that connect OSGM to existing branches of optimization theory and practice.

==> sec_practical_algo.tex <==
\subsection{Two practical variants of {\ohb}}

In this section, we propose two variants of {\ohb} that are both observed to perform well in practice. 
One variant uses the lookahead landscape action, tailored to heavy-ball feedback, to suppress the regret and hence accelerate the convergence;  the other variant uses the advanced online learning algorithm {\adagrad} to reduce the regret and accelerate the convergence. While the lookahead variant yields the best results in theory, the {\adagrad} variant requires fewer calls to the gradient oracle and works equally well (\Cref{sec:exp}).

\subsubsection{{\ohblook}}
Part I \cite{gao2025gradient} introduced the lookahead landscape action, which takes an additional gradient step on the proposed iterate $x^{k + 1 / 2}$ to suppress the regret of online gradient descent on feedback. 
Since the heavy-ball feedback is defined with respect to the potential function, the additional gradient step needs to be
taken with respect to the potential function $\varphi_{\omega}(\cdot, ~ z_2^{k + 1 / 2})$ as well. 
As a result, the lookahead landscape action for {\ohb} is
\begin{align}
  \Mlook (z^{k + 1 / 2}) & \assign ( z_1^{k + 1 / 2} - \tfrac{1}{L +
  \omega} \nabla_{1} \varphi_{\omega} (z^{k + 1 / 2}), ~ z_2^{k + 1 / 2} ) \nonumber\\
  & = ( z_1^{k + 1 / 2} - \tfrac{1}{L + \omega} [\nabla f (z^{k + 1 / 2}) +
  \omega (z_1^{k + 1 / 2} - z_2^{k + 1 / 2})], ~ z_2^{k + 1 / 2} ) \nonumber\\
  & = ( ( 1 - \tfrac{\omega}{L + \omega} ) z_1^{k + 1 / 2} +
  \tfrac{\omega}{L + \omega} z_2^{k + 1 / 2} - \tfrac{1}{L + \omega} \nabla f (z^{k + 1 / 2}), ~ z_2^{k + 1 / 2} ), \nonumber
\end{align}
where $\nabla_{1} \varphi_{\omega}(z)$ denotes the gradient with respect to $z_1$ and the stepsize is the inverse of the smoothness constant $L + \omega$ of the potential function $\varphi_{\omega}(z)$ with respect to $z_1$. 
{\ohblook} determines the next state $z^{k+1}$ by composing the lookahead and monotone landscape actions:
\[ z^{k + 1} = \Mmonolook(z^{k + 1 / 2}, ~ z^k) \assign \Mmono ( \Mlook(z^{k + 1 / 2}), ~ z^k ) . \]
\Cref{alg:ohblook} summarizes {\ohblook}, with monotone landscape action implemented by the null step.
The global convergence of {\ohblook} is established in \Cref{thm:ohblook}.

\begin{algorithm}[H]
  \caption{{\ohblook}\label{alg:ohblook}}
  \begin{algorithmic}[1]
  \Require{Initial state $z^1$ with $z_1^1 = z_2^1$, initial stepsize $P_1 \in \mathbb{R}^{n \times n}$ and momentum parameter $\beta_1 \in \mathbb{R}$, online gradient descent stepsizes $\eta_P$ and $\eta_{\beta}$}
  \For{$k = 1, 2, \dots$}
        \State $z^{k + 1 / 2} = ( z_1^k - P_k \nabla f (z^k) + \beta_k (z_1^k - z_2^{k}),~ z_1^k )$
          \Comment{State proposal from scheduler}
        \vspace{0.25\baselineskip}
        \State $z_{\text{look}}^{k + 1} = (z_1^{k + 1 / 2} -\tfrac{1}{L + \omega} \nabla_{1} \varphi_{\omega} (z^{k + 1 / 2}),~ z_2^{k+1/2} )$
          \Comment{Lookahead action}
        \vspace{0.25\baselineskip}
        \State $z^{k+1} = \argmin \{ \varphi_{\omega} ( z_{\text{look}}^{k+1}), \varphi_{\omega} (z^k) \}$
          \Comment{Monotone action by null step}
        \vspace{0.25\baselineskip}
        \State $P_{k + 1} = P_k - \eta_P \nabla_P h_{z^k} (P_k, \beta_k)$
          \Comment{Online gradient update on $P$}
        \vspace{0.25\baselineskip}
        \State $\beta_{k + 1} = \beta_k - \eta_{\beta} \nabla_{\beta} h_{z^k} (P_k, \beta_k)$
          \Comment{Online gradient update on $\beta$}
        \vspace{0.25\baselineskip}
  \EndFor
\end{algorithmic}
\end{algorithm}

\begin{thm}[Global convergence] \label{thm:ohblook}
  Suppose $f$ is $L$-smooth and convex. Choose the parameters $\omega = 3 L$, $\tau = 16 L^2$, $\eta = \tfrac{\tau}{2 L^2 (L + \omega)}$, and online gradient stepsizes $\eta_P = \tfrac{\eta_{\beta}}{L^2} = \eta$.
  % $\tau \geq \max \{ 2 L^2, 2 L \omega \}$. 
  % Then {\ohblook} satisfies
  % \begin{align}
  %   f (x^{K + 1}) - f^{\star} & \leq \tfrac{f (x^1) - f^{\star}}{K V
  %   \max \{ \frac{1}{K} \textstyle \sum_{k = 1}^K - h_{z^k} (\hat{P}, \hat{\beta}) - \frac{L^2 (L + \omega)}{\tau K} \| (P_1 - \hat{P}, \beta_1 -
  %   \hat{\beta}) \|^2, 0 \} + 1}, \tag{convex}\\
  %   f (x^{K + 1}) - f^{\star} & \leq [f (x^1) - f^{\star}] ( 1 -
  %   \mu \max \{ \tfrac{1}{K} \textstyle \sum_{k = 1}^K - h_{z^k} (\hat{P},
  %   \hat{\beta}) - \tfrac{L^2 (L + \omega)}{\tau K} \| (P_1 - \hat{P}, \beta_1
  %   - \hat{\beta}) \|^2, 0 \}  )^K . \tag{$\mu$-strongly convex}
  % \end{align}
  % where $V$ and $\Delta$ are constants defined in \Cref{thm:heavyball-reduction}.
  % In particular, if $\omega = 3 L$ and $\tau = 16 L^2$, 
  Then {\ohblook} converges globally at rate:
  \begin{align}
    f (z^{K + 1}) - f^{\star} & \leq \tfrac{f (z^1) - f^{\star}}{K V
    \max \{ \frac{1}{8 L} - \frac{L}{4 K} \| ( P_1
    - \frac{1}{4 L} I, \beta_1 - \frac{1}{2} ) \|^2, 0 \} +
    1}, \tag{convex}\\
    f (z^{K + 1}) - f^{\star} & \leq [f (z^1) - f^{\star}] ( 1 -
    \mu \max \{ \tfrac{1}{8 L} - \tfrac{L}{4 K} \| (
    P_1 - \tfrac{1}{4 L} I, \beta_1 - \tfrac{1}{2} ) \|^2, 0
    \}  )^K, \tag{$\mu$-strongly convex}
  \end{align}
  where $V$ and $\Delta$ are constants defined in \Cref{thm:heavyball-reduction}.
\end{thm}

\begin{rem}
Asymptotically, {\ohblook} converges with complexity $\Ocal(1/\varepsilon)$ for convex objectives and $\Ocal(\kappa \log(1/\varepsilon))$ complexity for strongly convex functions.
\end{rem}

\subsubsection{{\ohbada}}

An alternative variant replaces online
gradient descent by {\adagrad}.
%This variant can be viewed as {\ogd} with coordinate-wise adaptive stepsizes that decrease the regret.
\Cref{alg:ohbada} presents the algorithm {\ohbada}, with monotone landscape action implemented by the null step.
{\adagrad} maintains the cumulative square of feedback gradients $U_k$
and $v_k$ in \cref{line:ohbada-U,line:ohbada-v} and revises {\ogd} as in \cref{line:ohbada-P,line:ohbada-beta}. The global convergence of
{\ohbada} is established in \Cref{thm:ohbada} below.

\begin{algorithm}[H]
  \caption{{\ohbada}\label{alg:ohbada}}
  \begin{algorithmic}[1]
  \Require{Initial state $z^1$ with $z_1^1 = z_2^1$, initial $U_1 = \mathbf{0}$ and $v_1 = 0$, initial stepsize $P_1 \in \Pcal$ and $\beta_1 \in \Bcal$, {\adagrad} stepsizes $\eta_P$ and $\eta_{\beta}$}
  \For{$k = 1, 2, \dots$}
    \State $z^{k + 1 / 2} = ( z_1^k - P_k \nabla f (z^k) + \beta_k (z_1^k - z_2^{k}), ~ z_1^k )$
          \Comment{State proposal from scheduler}
      \vspace{0.25\baselineskip}
    \State $z^{k+1} = \argmin \{ \varphi_\omega (z^{k + 1 / 2}), \varphi_\omega (z^k) \}$
      \Comment{Monotone action by null step}
      \vspace{0.25\baselineskip}
    \State $U_{k + 1} = U_k + \nabla_P h_{z^k} (P_k, \beta_k) \circ  \nabla_P h_{z^k} (P_k, \beta_k)$ \label{line:ohbada-U}
      \Comment{Cumulative gradient square of $P$}
      \vspace{0.25\baselineskip}
    \State $v_{k + 1} = v_k + \nabla_{\beta} h_{z^k} (P_k, \beta_k) \circ \nabla_{\beta} h_{z^k} (P_k, \beta_k)$ \label{line:ohbada-v}
      \Comment{Cumulative gradient square of $\beta$}
      \vspace{0.25\baselineskip}
    \State $U^{-1/2}_{k+1} = \tfrac{1}{\sqrt{U_{k + 1}}}$
      \Comment{Elementwise inverse square root}
    \State $P_{k + 1} = \Pi_{\mathcal{P}} [P_k - \eta_P U^{-1/2}_{k+1} \circ \nabla_P h_{z^k} (P_k, \beta_k)]$ \label{line:ohbada-P}
      \Comment{{\adagrad} update on $P$}
      \vspace{0.25\baselineskip}
    \State $\beta_{k + 1} = \Pi_{\mathcal{B}} [\beta_k - \eta_{\beta} v^{- 1 / 2}_{k +1} \nabla_{\beta} h_{z^k} (P_k, \beta_k)]$ \label{line:ohbada-beta}
      \Comment{{\adagrad} update on $\beta$}
    \vspace{0.25\baselineskip}
  \EndFor
\end{algorithmic}
\end{algorithm}

\begin{thm}[Global convergence of {\ohbada}] \label{thm:ohbada}
  Suppose $f$ is $L$-smooth convex and both the candidate sets $\Pcal$ and $\Bcal$ are bounded. For any benchmark stepsize and momentum $(\hat{P},
  \hat{\beta}) \in \mathcal{P} \times \mathcal{B}$, {\ohbada} with $\eta_P = \eta_{\beta}$ converges globally at rate:
  \begin{align}
    f (z^{K + 1}) - f^{\star} & \leq \tfrac{f (z^1) - f^{\star}}{K V
    \max \{ \frac{1}{8 L} - \frac{\rho_K (\hat{P}, \hat{\beta})}{K}, 0
    \} + 1} ; \tag{convex}\\
    f (z^{K + 1}) - f^{\star} & \leq [f (z^1) - f^{\star}] ( 1 -
    \mu \max \{ \tfrac{1}{8
    L} - \tfrac{\rho_K (\hat{P}, \hat{\beta})}{K}, 0 \}  )^K,
    \tag{$\mu$-strongly convex}
  \end{align}
  where $\rho_K (\hat{P}, \hat{\beta}) =\mathcal{O} ( \sqrt{K} )$ is the regret of {\adagrad}.
\end{thm}


